Learning Attention-based Representations from Multiple Patterns for Relation Prediction in Knowledge Graphs

Knowledge bases, and their representations in the form of knowledge graphs (KGs), are naturally incomplete. Since scientific and industrial applications have extensively adopted them, there is a high demand for solutions that complete their information. Several recent works tackle this challenge by learning embeddings for entities and relations, then employing them to predict new relations among the entities. Despite their aggrandizement, most of those methods focus only on the local neighbors of a relation to learn the embeddings. As a result, they may fail to capture the KGs' context information by neglecting long-term dependencies and the propagation of entities' semantics. In this manuscript, we propose {\AE}MP (Attention-based Embeddings from Multiple Patterns), a novel model for learning contextualized representations by: (i) acquiring entities' context information through an attention-enhanced message-passing scheme, which captures the entities' local semantics while focusing on different aspects of their neighborhood; and (ii) capturing the semantic context, by leveraging the paths and their relationships between entities. Our empirical findings draw insights into how attention mechanisms can improve entities' context representation and how combining entities and semantic path contexts improves the general representation of entities and the relation predictions. Experimental results on several large and small knowledge graph benchmarks show that {\AE}MP either outperforms or competes with state-of-the-art relation prediction methods.

==> sec/ablation123-tab.tex <==
\begin{table}[h]
\centering
\caption{Ablation studies parametrization settings.}
\label{tab:ablationhp}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{llll}
\toprule
\multirow{2}{*}{Hyperparamter} & \multicolumn{3}{c}{Ablation Studies} \\ \cline{2-4} 
 & \multicolumn{1}{c|}{\textit{(i)}} & \multicolumn{1}{c|}{(ii)} & \multicolumn{1}{c}{\textit{(iii)}} \\ \hline
\multicolumn{1}{l|}{Batch size} & \multicolumn{1}{l|}{128} & \multicolumn{1}{l|}{128} & 128 \\
\multicolumn{1}{l|}{Epoch} & \multicolumn{1}{l|}{20} & \multicolumn{1}{l|}{10} & 5 \\
\multicolumn{1}{l|}{Hidden state dimension} & \multicolumn{1}{l|}{128} & \multicolumn{1}{l|}{128} & 128 \\
\multicolumn{1}{l|}{L2 regularization weight} & \multicolumn{1}{l|}{$10^{-7}$} & \multicolumn{1}{l|}{$10^{-7}$} & $10^{-7}$ \\
\multicolumn{1}{l|}{Learning rate} & \multicolumn{1}{l|}{$10^{-3}$} & \multicolumn{1}{l|}{$10^{-3}$} & $10^{-3}$ \\
\multicolumn{1}{l|}{Maximum entities context hops} & \multicolumn{1}{l|}{3} & \multicolumn{1}{l|}{\{1,2,3\}} & 3 \\
\multicolumn{1}{l|}{Maximum semantic path length} & \multicolumn{1}{l|}{3} & \multicolumn{1}{l|}{\{1,2,4\}} & 3 \\
\multicolumn{1}{l|}{Random attention context selection criteria} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & 0.2 \\
\bottomrule
\end{tabular}%
% }

==> sec/bckup.tex <==
BCKUP


LOCAL
% \begin{equation}
%     \alpha_{ek}^{local} = \textrm{softmax}_{e}(s_{e}^{k}) = \frac{\textrm{exp}(s_{e}^{k})}{\sum_{e' \in \mathcal{N}_{E}}\textrm{exp}(s_{e'}^{k})}
% \end{equation}

% \begin{equation}
%     {s^{local}}_{e}^{k} = \alpha_{ek}^{local} * s_{e}^{k}
% \end{equation}

% \begin{subequations}\label{eq:localatt}
%     \begin{minipage}{0.5\textwidth}\label{eq:localatta}
%         \begin{align}
%         \alpha_{rk}^{local} = \textrm{softmax}_{r}(s_{r}^{k}) = \frac{\textrm{exp}(s_{r}^{k})}{\sum_{r' \in \mathcal{N}_{R}}\textrm{exp}(s_{r'}^{k})}
%         \end{align}
%     \end{minipage}
%     \begin{minipage}{0.5\textwidth}\label{eq:localatta}
%         \begin{align}
%         {s^{local}}_{r}^{k} = \sigma(\sum_{r \in \mathcal{N}_{R}}\alpha_{rk}^{local} Ws_{r}^{k})
%         \end{align}
%     \end{minipage}
% \end{subequations}

\begin{subequations}\label{eq:localatt}
    \begin{minipage}{0.5\textwidth}\label{eq:localatta}
        \begin{align}
        \alpha_{rk}^{local} = \textrm{align}_{r}(s^{k}, s_{r}^{k}) = \frac{\textrm{exp}({s^{k}}^\intercal \weights s_{r}^{k})}{\sum_{r' \in \mathcal{N}_{R}}\textrm{exp}({s^{k}}^\intercal \weights s_{r'}^{k}))}
        \end{align}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}\label{eq:localatta}
        \begin{align}
        {s^{local}}_{r}^{k} = \sigma(\sum_{r \in \mathcal{N}_{R}}\alpha_{rk}^{local} \weights s_{r}^{k})
        \end{align}
    \end{minipage}
\end{subequations}

GLOBAL
% \begin{equation}
%     \alpha_{ek}^{global} = \textrm{softmax}_{k}(s_{e}^{k}) = \frac{\textrm{exp}(s_{e}^{k})}{\sum_{i \in \mathcal{N}_{I}}\textrm{exp}(s_{e}^{i})}
% \end{equation}

% \begin{equation}
%     {s^{global}}_{e}^{k} = \alpha_{ek}^{local} * s_{e}^{k}
% \end{equation}

% \begin{subequations}\label{eq:globalatt}
%     \begin{minipage}{0.5\textwidth}\label{eq:globalatta}
%         \begin{align}
%         \alpha_{rk}^{global} = \textrm{softmax}_{k}(s_{r}^{k}) = \frac{\textrm{exp}(s_{r}^{k})}{\sum_{i \in \mathcal{N}_{I}}\textrm{exp}(s_{r}^{i})}
%         \end{align}
%     \end{minipage}
%     \begin{minipage}{0.5\textwidth}\label{eq:globalattb}
%         \begin{align}
%         {s^{global}}_{r}^{k} = \sigma(\sum_{i \in \mathcal{N}_{I}}\alpha_{ri}^{global} * s_{r}^{i})
%         \end{align}
%     \end{minipage}
% \end{subequations}

\begin{subequations}\label{eq:globalatt}
    \begin{minipage}{0.5\textwidth}\label{eq:globalatta}
        \begin{align}
        \alpha_{rk}^{global} = \textrm{align}_{k}(s_{r}, s_{r}^{k}) = \frac{\textrm{exp}({s_{r}}^\intercal \weights s_{r}^{k})}{\sum_{i \in \mathcal{N}_{I}}\textrm{exp}({s_{r}}^\intercal \weights s_{r}^{i})}
        \end{align}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}\label{eq:globalattb}
        \begin{align}
        {s^{global}}_{r}^{k} = \sigma(\sum_{i \in \mathcal{N}_{I}}\alpha_{ri}^{global} \weights s_{r}^{i})
        \end{align}
    \end{minipage}
\end{subequations}

RANDOM
% \begin{equation}
%     \alpha_{ek}^{random} = \textrm{softmax}_{ek}(s_{e}^{k}) = \frac{\textrm{exp}(s_{e}^{k})}{\sum_{\{i,e'\} \in \mathcal{N}_{R}}\textrm{exp}(s_{e'}^{i})}
% \end{equation}

% \begin{equation}
%     {s^{random}}_{e}^{k} = \alpha_{ek}^{local} * s_{e}^{k}
% \end{equation}

% \begin{subequations}\label{eq:randomatt}
%     \begin{minipage}{0.5\textwidth}\label{eq:randomatta}
%         \begin{align}
%         \alpha_{rk}^{random} = \textrm{softmax}_{rk}(s_{r}^{k}) = \frac{\textrm{exp}(s_{r}^{k})}{\sum_{\{i,r'\} \in \mathcal{N}_{R}}\textrm{exp}(s_{r'}^{i})}
%         \end{align}
%     \end{minipage}
%     \begin{minipage}{0.5\textwidth}\label{eq:randomattb}
%         \begin{align}
%         {s^{random}}_{r}^{k} = \sigma(\sum_{\{i,r\} \in \mathcal{N}_{R}}\alpha_{ri}^{random} * s_{r}^{i})
%         \end{align}
%     \end{minipage}
% \end{subequations}

\begin{subequations}\label{eq:randomatt}
    \begin{minipage}{0.5\textwidth}\label{eq:randomatta}
        \begin{align}
        \alpha_{rk}^{random} = \textrm{align}_{rk}(s, s_{r}^{k}) = \frac{\textrm{exp}(s^\intercal \weights s_{r}^{k})}{\sum_{\{i,r'\} \in \mathcal{N}_{R}}\textrm{exp}(s^\intercal \weights s_{r'}^{i})}
        \end{align}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}\label{eq:randomattb}
        \begin{align}
        {s^{random}}_{r}^{k} = \sigma(\sum_{\{i,r\} \in \mathcal{N}_{R}}\alpha_{ri}^{random} \weights s_{r}^{i})
        \end{align}
    \end{minipage}
\end{subequations}

DATASET STATISTICS
\begin{table*}[t]
\centering
\caption{Datasets statistical summary.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccccccc@{}}
\toprule
 &  &  &  &  & \multicolumn{5}{c}{Entities} & \multicolumn{5}{c}{Relations} \\
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{Edges} & \multicolumn{2}{c}{\#} & \multicolumn{3}{c|}{Entities degree} & \multicolumn{2}{c}{\#} & \multicolumn{3}{c}{Relations degree} \\ \cmidrule(l){2-15} 
\multicolumn{1}{c|}{Dataset} & Training & Validation & Test & \multicolumn{1}{c|}{Total} & Total & Unique & Mean & Median & \multicolumn{1}{c|}{Std} & Total & Unique & Mean & Median & Std \\ \midrule
% \multicolumn{1}{c|}{\textit{DDB14}} & 36561 & 4000 & 4000 & \multicolumn{1}{c|}{44561} & 9203 & 468 & 9,684 & 5 & \multicolumn{1}{c|}{383,322} & 14 & 0 & 500,5 & 3182,92857 & 7105,17718 \\
% \multicolumn{1}{c|}{\textit{NELL995}} & 137465 & 5000 & 5000 & \multicolumn{1}{c|}{147465} & 63917 & 32137 & 4,6142 & 1 & \multicolumn{1}{c|}{29,4024} & 198 & 0 & 368 & 744,7727 & 1316,1541 \\
\multicolumn{1}{c|}{\textit{WN18}} & 141442 & 5000 & 5000 & \multicolumn{1}{c|}{151442} & 40943 & 5 & 7,3976 & 4 & \multicolumn{1}{c|}{16,4639} & 18 & 0 & 8413,4444 & 3242,5 & 12336,0782 \\
\multicolumn{1}{c|}{\textit{WN18RR}} & 86835 & 3134 & 3034 & \multicolumn{1}{c|}{93003} & 40943 & 5754 & 4,543 & 3 & \multicolumn{1}{c|}{8,5753} & 11 & 0 & 8454,8181 & 3150 & 12540,08 \\
\multicolumn{1}{c|}{\textit{FB15k}} & 483142 & 59071 & 50000 & \multicolumn{1}{c|}{592213} & 14951 & 21 & 79,2205 & 50 & \multicolumn{1}{c|}{220,7223} & 1345 & 115 & 440,307 & 26 & 1565,1318 \\
\multicolumn{1}{c|}{\textit{FB15k-237}} & 272115 & 20466 & 17535 & \multicolumn{1}{c|}{310116} & 14541 & 314 & 42,654 & 260 & \multicolumn{1}{c|}{127,7005} & 237 & 0 & 1308,5063 & 426 & 2467,0039 \\ \bottomrule
\end{tabular}%
}

==> sec/intro_v0.tex <==
\vspace{-0.2cm}
Humankind knowledge processed by machines can be posed as sets of information (\textit{i.e.}, facts, beliefs, and rules) circa entities. By connecting these sets of information and their relationships, we are able to build a network of knowledge. Knowledge bases~(KBs) play a fundamental role in compiling this network of knowledge, structuring and storing information, its properties, and its relationships.

Existing compiled KBs such as WordNet~\cite{miller1995wordnet} and Freebase~\cite{bollacker2008freebase} organize open information over topological and non-topological relations. They have succeeded as core resources on knowledge-related tasks such as question answering~\cite{yih2015qa},  query expansion~\cite{dalton2014qexp}, information retrieval~\cite{liu2018entity}, recommender systems~\cite{palumbo2017entity2rec}, and even commonsense reasoning~\cite{lin2019kagnet}. Typically, the information in these bases are organized according to a conceptual structure in the form of triples \mbox{$(head, relation, tail)$}, in which $head$ and $tail$ are entities (also called \textit{subject} and \textit{object}, respectively) and $relation$ (also called \textit{predicate}) is the relationship between both entities that qualifies the triple semantics. A common representation of KBs is the labeled multi-digraph. The labeled multi-digraph are graphs whose edges have an associated direction (directed graphs, digraphs) and an associated label (labeled digraphs), and whose nodes might have multiple directed edges between them (multi-digraph). In this representation, also commonly called as Knowledge Graphs~(KGs) within the KBs domain, the nodes are the entities ($head$ and $tail$), the edges express relationships between entities, and the edges' labels define the semantics of each relationship ($relation$).

Despite the success of KGs as core resources on a large plethora of tasks, real-world KGs usually experience incompleteness and noisy information. They are strictly dependable on new information acquisition, which is often hard to obtain and noisy prone once the information continuously evolves over time~\cite{levesque1984ikb}. Thus, an essential aspect regarding KGs arises: the existence of automatic methods to complete their information. This capacity involves solving the prediction of missing relations among entities in the KG.

Several previous works have proposed techniques to predict and infer new relationships from the existing information to address the capabilities of completing knowledge graphs. Such methods have been mostly driven by the recent advances in learning representations of symbolic data and can be roughly divided into two categories~\cite{dumancic2019srl}: distributional~\cite{bordes2013transe,trouillon2016complex,sun2018rotate,zhang2019quate} and symbolic methods~\cite{galarraga2015amie,wang2016knowledge}. The distributional methods aim to learn and operate latent representations, \ie{}, embedding vectors, of entities and relations. These methods rely on encoding the interactions between entities' neighborhood, \textit{i.e.}, the entities' local relationships, into low-dimensional dense vectors, which allow for new relationships between entities to be predicted from interactions of the entities' embeddings~\cite{nickel2016kge}. Differently, the symbolic methods~\cite{galarraga2015amie,wang2016knowledge} aim to predict new relations from the observed examples in the knowledge graph. Generally, these methods extract rules from the examples in order to model logical patterns, \ie{}, semantic paths between entities~\cite{nickel2016kge}. Methods grounded in the symbolic paradigm can reason over complex relational paths due to their rule-based grounding. However, they are well-known for suffering from scalability issues, which limit their rule-inference search space, consequently, their relation prediction capabilities. In contrast, the embedding-based methods (grounded in the distributional paradigm) are capable of only learning local structures, requiring further enhancements to allow for more generality. Nonetheless, they scale, being capable of operating on knowledge graphs with millions of facts.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{img/kg_example2-small.png}
    \vspace{-0.7cm}
    \caption{Example of a knowledge graph. Gray circles indicate the head and tail entities. Dashed-arrows are potentially missing relations. Yellow-shaded arrows indicate the semantic paths between the head and tail. Green, red, and blue-shaded areas represent the different attention mechanisms used in \ourmodel{}.}
    \label{fig:example}
    \vspace{-0.7cm}
\end{figure}

Motivated by the aforementioned observations, we address in this work the relation prediction challenge to complete knowledge bases designing a novel embedding-based model called \ourmodel{}~(\textbf{A}ttention-based \textbf{E}mbeddings from \textbf{M}ultiple \textbf{P}atterns). \ourmodel{} aims at the major advantages of each paradigm: local structure learning and scalability from the distributional paradigm and generality with semantic paths from the symbolic paradigm. To achieve such a goal \ourmodel{} addresses learning contextualized representations from the combination of entities context and semantic paths. The key insights of \ourmodel{} are based on the perception that multiple patterns exist to relate entities. Similar to a word in a sentence, entities' local neighborhood evidences their structure and properties, while semantic paths relate long-term dependencies among them. Besides, the unification of these contextual information provides enhanced information to predict new relations among existing entities in knowledge graphs. Figure~\ref{fig:example} exemplifies the patterns and mechanisms that \ourmodel{} uses to learn representations. Primarily, \ourmodel{} operates an attention-enhanced message-passing scheme, which iteratively propagates the $k$-hop local neighbor information of a given entity over the neighborhood edges, paying attention in local (Figure~\ref{fig:example} red-shaded areas, where light red is the local 1-hop neighbors and the dark red is the local 2-hop neighbors), global (Figure~\ref{fig:example} green area), and random (Figure~\ref{fig:example} blue area) aspects of the neighborhood to learn a unique contextualized representation of the given entity and its neighborhood. Secondly, \ourmodel{} identifies the semantic paths between a pair of entities and combine them into a single semantic path representation (Figure~\ref{fig:example} yellow arrows). Finally, our model combines both contextualized entities and semantic path representations in order to inform the probability of a new relationship between a pair of entities.

Therefore, we summarize as the main contributions of this paper:
\begin{enumerate}\vspace{-0.25cm}
    \item[i)] A novel attention-enhanced message-passing scheme for learning contextualized entities representations;\vspace{-0.25cm}
    \item[ii)] Identification of semantic paths between a pair of entities and the combination of the paths' representations into a single general semantic path representation; and\vspace{-0.25cm}
    \item[iii)] Combination of contextualized entities representations and semantic path representations for relation prediction.\vspace{-0.25cm}
\end{enumerate}

We conduct an extensive evaluation of \ourmodel{} on the main knowledge graphs benchmarks (WN18~\cite{bordes2013transe}, WN18RR~\cite{dettmers2017wn18rr}, FB15k~\cite{bordes2013transe}, and FB15k-237~\cite{toutanova2015fb15k237}). We compare the efficiency of our model against some state-of-the-art models in relation prediction. Our experimental protocol considers the mean reciprocal rank (MRR), mean rank (MR), and hit ratio at $k$ (Hit@$k$) metrics. The metrics results show that \ourmodel{} outperforms the compared methods in three (WN18, WN18RR, and FB15k) out of the four datasets and demonstrates competitive results on the fourth benchmark.
